Type-Directed Code Reuse using Integer Linear Programming

In many common scenarios, programmers need to implement functionality that is already provided by some third party library. This paper presents a tool called Hunter that facilitates code reuse by finding relevant methods in large code bases and automatically synthesizing any necessary wrapper code. The key technical idea underlying our approach is to use types to both improve search results and guide synthesis. Specifically, our method computes similarity metrics between types and uses this information to solve an integer linear programming (ILP) problem in which the objective is to minimize the cost of synthesis. We have implemented Hunter as an Eclipse plug-in and evaluate it by (a) comparing it against S6, a state-of-the-art code reuse tool, and (b) performing a user study. Our evaluation shows that Hunter compares favorably with S6 and significantly increases programmer productivity.

==> prev-intro.tex <==

\section{Previous Introduction}

In many common scenarios, programmers need to implement functionality that is already provided by some third party library. In such cases, accepted wisdom dictates that it is preferable to reuse existing software components rather than reimplementing the desired functionality from scratch. Indeed, there are at least two benefits to software reuse: First, utilizing existing components significantly increases programmer  productivity, allowing developers to focus on more creative tasks. Second, implementations provided by existing APIs are typically well-tested; hence, reusing existing components reduces the likelihood that the implementation is buggy. 

Unfortunately, there is often a wide gap between the adage ``software reuse is good" and the actual reality of software development: More often than not,  programmers end up reimplementing a functionality that already exists somewhere. This duplicated effort is sometimes inadvertent, as programmers may not know whether the desired functionality exists or which third-party library provides it. In other cases, the exposed interface may not quite fit the developer's needs, tempting programmers to reimplement the desired functionality rather than performing the tedious task of writing ``wrapper" or ``adapter" code. 

This paper seeks to address both of these problems by automatically synthesizing adapter methods from input-output examples and method signatures. 
Specifically, given some test cases and a method signature, our tool \system searches existing code repositories to find relevant software components and synthesizes any wrapper code needed to invoke the existing interface. Hence, our approach allows programmers to reuse existing software without even knowing that they are reusing it and saves them from the prosaic task of %searching for relevant methods and  
writing tedious wrapper code.

At a technical level, there are three key components underlying our approach: 
 
\begin{enumerate}
\item {\bf \emph{Code search:}}  We first identify a set of candidate \emph{adaptee methods} by performing \emph{$k$-nearest neighbor search} over the database of existing software components. Our technique uses a combination of method signatures and natural language comments to map each software component to a vector in $n$-dimensional space.
\item {\bf \emph{Interface alignment:}} Given a candidate adaptee with signature $\sig$ and a  \emph{penalty matrix} estimating the cost of converting a type $\tau$ to anther type $\tau'$, our algorithm finds a lowest-cost mapping between parameters of $\sig$ and those of the desired signature $\sig'$. We refer to this problem as \emph{interface alignment} and solve it using integer linear programming (ILP).
%  in which the goal is to minimize the total cost of $\Sigma_{ij} f(i, j)$ where f is a function estimating the cost of converting parameter i of S to parameter j of S’.
\item {\bf \emph{Code synthesis:}} Given a candidate alignment between the desired method $\mathcal{M'}$ and a candidate adaptee $\mathcal{M}$, we need to generate wrapper code that performs any necessary type conversions.  We formulate this code synthesis task as the reachability problem in Petri nets and synthesize code by following a sequence of transitions that satisfy certain semantic conditions.

\end{enumerate}
 

Figure~\ref{fig:hunter} gives a schematic overview of our approach. The input to our system consists of a set of test cases and a user query, which includes the name and signature of the method to synthesize as well as any comments describing its functionality. Our method starts by performing \emph{code search} over a large corpus of existing software  and identifies a  method $\adaptee$ that most closely matches the user's query.
Given such a candidate adaptee $\adaptee$, the \emph{interface alignment} and \emph{code synthesis} modules work together to synthesize 
a new method $\adaptee'$ that ``adapts" $\adaptee$ to fit the desired interface. Our approach does not modify the underlying implementation of method $\adaptee'$, but rather synthesizes adapter code to perform any necessary pre- and post-processing steps. 


While the code synthesized by our approach is always guaranteed to type-check and satisfy certain semantic constraints,  it may or may not be the program that the user intended. To increase our confidence about the correctness of the synthesized program, we run it on  test cases provided by the user and \emph{backtrack}  if any test fails. In our approach, there are three possible forms of backtracking: (i) identifying a new adaptee from the database, (ii) finding a different solution to the interface alignment problem, or (iii) synthesizing different adapter code by finding a new path in the corresponding Petri net. The algorithm repeats this \emph{search-align-synthesize-and-check} loop until the candidate program passes all test cases provided by the user.

%In this context, backtracking involves either retrieving a different candidate method from the database, finding a different solution to the interface alignment problem, or 
%synthesizing a different code snippet for performing type conversion. 

We have implemented the proposed approach in a tool called \system \ and used it to synthesize XXX non-trivial programs taken from real Java codebases and algorithms textbooks. Our evaluation shows that \system \ is both useful and practical: In XXX\% of the cases, our approach was able to synthesize the correct program and took less than XXX seconds on average to return the desired implementation.

To summarize, this paper makes the following contributions:

\begin{itemize}
\item We propose a database-driven approach for automatically synthesizing adapter methods from signatures, comments, and test cases.
\item We describe a novel \emph{semantic code search} algorithm that utilizes both method signatures and  implementations.
\item We define the \emph{interface alignment problem} for matching a pair of method signatures and show how it can be solved using integer linear programming (ILP).
\item We show how Petri nets can be used for performing type-directed program synthesis. Specifically,   given a pair of types $(\tau_\emph{in}, \tau_\emph{out})$, we formulate the problem of converting objects of type $\tau_\emph{in}$ to objects of type $\tau_\emph{out}$ as a reachability problem in Petri nets.
\item We describe an implementation of our approach in a tool called \system \ and use it to succesfully synthesize non-trivial programs taken from real-world Java software and algorithms textbooks.
\end{itemize} 

